Multi-Electrostatic FPGA Placement Considering SLICEL-SLICEM Heterogeneity, Clock Feasibility, and Timing Optimization

When modern FPGA architecture becomes increasingly complicated, modern FPGA placement is a mixed optimization problem with multiple objectives, including wirelength, routability, timing closure, and clock feasibility. Typical FPGA devices nowadays consist of heterogeneous SLICEs like SLICEL and SLICEM. The resources of a SLICE can be configured to {LUT, FF, distributed RAM, SHIFT, CARRY}. Besides such heterogeneity, advanced FPGA architectures also bring complicated constraints like timing, clock routing, carry chain alignment, etc. The above heterogeneity and constraints impose increasing challenges to FPGA placement algorithms. In this work, we propose a multi-electrostatic FPGA placer considering the aforementioned SLICEL-SLICEM heterogeneity under timing, clock routing and carry chain alignment constraints. We first propose an effective SLICEL-SLICEM heterogeneity model with a novel electrostatic-based density formulation. We also design a dynamically adjusted preconditioning and carry chain alignment technique to stabilize the optimization convergence. We then propose a timing-driven net weighting scheme to incorporate timing optimization. Finally, we put forward a nested Lagrangian relaxation-based placement framework to incorporate the optimization objectives of wirelength, routability, timing, and clock feasibility. Experimental results on both academic and industrial benchmarks demonstrate that our placer outperforms the state-of-the-art placers in quality and efficiency.

==> doc/answer.tex <==
{
\onecolumn
\normalsize

\ \\
\textbf{Responses to the reviewers}

\ \\
\textbf{Reviewer 1}
\begin{description}\itemsep.8em
\item[R1C1]
\textbf{
The paper considers the legalization problem in designs where cells can occupy multiple row heights, though the experimental results show only double row heights. The paper proposes two heuristics: one is based on chain movements and the other one is legalization while preserving the order. \\
Overall, the paper feels a bit unready in the sense that the two heuristics do not establish themselves clearly in terms of their applicability and their ability to fully legalize a placement because [12] is still needed.
}
\item[R1A1]
Thanks very much for the comments.

\item[R1C2]
\textbf{
- the chain movement algorithm does not guarantee legality, so as a result algorithm from [12] is used to fix placement, which is funny given that the proposed algorithm is supposed for detailed placement.
}
\item[R1A2]
{\color{blue}{
That is really a concern. 
If the input design is legal, the chain move algorithm can maintain legality, as mentioned in Section~\ref{sec:ndp}. 
Maybe we can run two flows. 
One is chain move + \cite{PLACE_DAC2016_Chow} + double-row placement; 
the other is \cite{PLACE_DAC2016_Chow} + chain move + double-row placement. 
Then compare the quality of two flows. 
But it might be better to do it in journal extension. 
}}

\item[R1C3]
\textbf{
- ordered double-row placement is introduced as some sort of post-processing step that is done in the last step of Algorithm 1. If that algorithm is doing what it is supposed to do (i.e., legalization), should it not be used in lieu of [12] to clean up the results from the chain movement algorithm?
}
\item[R1A3]
In general the algorithm can also be applied to resolve small amount of overlaps for legalization, 
but the computation effort turns out to an issue for layouts with large amount of overlaps due to its quadratic relation with maximum displacement. 
Therefore, we adopt it as an incremental optimization technique for legal designs. 
We have added this in the last paragraph of Section~\ref{sec:ext_to_typical_case}. 

\item[R1C4]
\textbf{
- The ordered double row placement can be considered as heuristic or optimal depending on the cell order case. It would have better if the authors outlined the complexity of the problem in the general case. Also, how does the algorithm behave, in terms of optimality, for the general case. 
}
\item[R1A4]
The general double-row placement problem without ordering constraints is very difficult, 
since the general single-row placement placement problem is already known as NP-hard \cite{PLACE_TCAD1989_Chowdhury}. 
We have added this in the last paragraph before Section~\ref{sec:nested_shortest_path}. 

\end{description}

\ \\
\textbf{Reviewer 2}
\begin{description}\itemsep.8em
\item[R2C1]
\textbf{
This paper proposes a multiple-row detailed placement of heterogeneous-sized cells. The proposed method consists of several steps including Chain move and
double-row placement. The efficiency of the proposed method is confirmed empirically.
}
\item[R2A1]
Thanks very much for the comments. 

\item[R2C2]
\textbf{
This method is interesting to the reviewer. But, the reviewer wonders whether the consistency is held during Ordered Double-Row Placement. For example, for the case in Fig. \ref{fig:double_row_place},
cell g and j are spread out of the rows. But, the movement of them seems to be free from the such irregularity. The reviewer would like to make it clear.
}
\item[R2A2]
In the case of Fig.~\subref*{fig:double_row_place3} where cells $e$, $g$, and $j$ spread out of the rows, 
their movements must keep the order within the two rows and not cause any overlap in the other rows. 
We have added this in the last paragraph before Section~\ref{sec:nested_shortest_path}. 

\end{description}

\ \\
\textbf{Reviewer 3}
\begin{description}\itemsep.8em
\item[R3C1]
\textbf{
The paper proposes procedures for detailed placement which includes multiple-row cells to optimize wire length and cell and pin density. The procedures include a new chain-based legalization, and a dynamic programming technique for improving wire length.
}
\item[R3A1]
Thanks very much for the comments. 

\item[R3C2]
\textbf{
Please include comparison with [12] in the simulation results as well as discuss in what ways this work is different or improves upon [12].
}
\item[R3A2]
{\color{blue}{
The work from \cite{PLACE_DAC2016_Chow} is a legalization algorithm that tries to remove overlaps with minimum displacement, 
while this work tries to optimize wirelength and density from globally placed designs. 
In general, a legalization algorithm that minimizes displacement usually degrades wirelength. 
It is not fair to compare our algorithm with \cite{PLACE_DAC2016_Chow}. 
It might be better to do it in journal extension. 
}}

\end{description}

\ \\
\textbf{Reviewer 4}
\begin{description}\itemsep.8em
\item[R3C1]
\textbf{
This paper proposes a detailed placement for multi-row heterogeneous-sized cells. The authors first optimize the wirelength, cell, and pin density for both single-row height cells and multi-row height cells. A nested dynamic programming based method is proposed for wirelength optimization. At last, they achieve good results compared with the recent work. \\
The results are good. And the method is also simple and reasonable.
}
\item[R3A1]
Thanks very much for the comments. 

\end{description}
}



==> figs/clock_penalty_2d.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\(\displaystyle \Gamma(\cdot)\) on x-axis direction},
x grid style={white!69.0196078431373!black},
xlabel={x},
xmajorgrids,
xmin=-3.3, xmax=3.30000000000001,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle \Gamma(\cdot)^x\)},
ymajorgrids,
ymin=-0.200000000000001, ymax=4.20000000000002,
ytick style={color=black}
]
\addplot [thick, red]
table {%
-3 4
-2.9 3.61
-2.8 3.24
-2.7 2.89
-2.6 2.56
-2.5 2.25
-2.4 1.96
-2.3 1.69
-2.2 1.44
-2.1 1.21
-2 0.999999999999998
-1.9 0.809999999999998
-1.8 0.639999999999998
-1.7 0.489999999999998
-1.6 0.359999999999998
-1.5 0.249999999999999
-1.4 0.159999999999999
-1.3 0.0899999999999991
-1.2 0.0399999999999994
-1.1 0.00999999999999966
-0.999999999999998 0
-0.899999999999998 0
-0.799999999999998 0
-0.699999999999998 0
-0.599999999999998 0
-0.499999999999998 0
-0.399999999999998 0
-0.299999999999998 0
-0.199999999999998 0
-0.0999999999999974 0
2.66453525910038e-15 0
0.100000000000003 0
0.200000000000003 0
0.300000000000003 0
0.400000000000003 0
0.500000000000003 0
0.600000000000003 0
0.700000000000003 0
0.800000000000003 0
0.900000000000003 0
1 1.26217744835362e-29
1.1 0.0100000000000006
1.2 0.0400000000000015
1.3 0.0900000000000026
1.4 0.160000000000003
1.5 0.250000000000004
1.6 0.360000000000005
1.7 0.490000000000006
1.8 0.640000000000007
1.9 0.810000000000007
2 1.00000000000001
2.1 1.21000000000001
2.2 1.44000000000001
2.3 1.69000000000001
2.4 1.96000000000001
2.50000000000001 2.25000000000002
2.6 2.56000000000002
2.7 2.89000000000002
2.80000000000001 3.24000000000002
2.90000000000001 3.61000000000002
3.00000000000001 4.00000000000002
};
\end{axis}

\end{tikzpicture}


==> texlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\geometry{twoside=true, head=12pt,
	paperwidth=9.2in, paperheight=11.8in,
	includeheadfoot, columnsep=1.8pc,
	top=45pt, bottom=45pt,
    left=51pt, right=51pt,
    %inner=54pt, outer=54pt,
	marginparwidth=1.8pc,heightrounded
}%
% \geometry{twoside=true, head=13pt,
	% paperwidth=8.5in, paperheight=11in,
	% includeheadfoot, columnsep=2pc,
	% top=45pt, bottom=55pt,
    % left=54pt, right=54pt,
    % %inner=54pt, outer=54pt,
	% marginparwidth=2pc,heightrounded
% }%
%\geometry{twoside=true, head=13pt,
%paperwidth=8.5in, paperheight=11in,
%includeheadfoot, columnsep=2pc,
%top=57pt, bottom=73pt, inner=54pt, outer=54pt,
%marginparwidth=2pc,heightrounded
%}%
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{soul}
\usepackage{graphicx}
\usepackage{amsmath}
% \usepackage{amssymb}
\newcommand\hmmax{0} % default 3
\newcommand\bmmax{0} % default 4
\usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
% \usepackage{algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
% \renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{siunitx}
\sisetup{product-units = single}

% ==== Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\bignorm}[1]{\left\lVert#1\right\rVert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\m}[1]{\mathbf{#1}}
\newcommand{\mx}{\m{x}}
\newcommand{\my}{\m{y}}
\newcommand{\mz}{\m{z}}
\newcommand{\bigmax}[2]{\max\left({#1}, {#2}\right)}
\newcommand{\bigmin}[2]{\min\left({#1}, {#2}\right)}
\newcommand{\bigparenthesis}[1]{\left({#1}\right)}
\newcommand{\bigbracket}[1]{\left[{#1}\right]}
\newcommand{\bigbrace}[1]{\left\{{#1}\right\}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}

% ==== Reference Style ========
\newcommand{\eqRef}[1]{Eq.~\eqref{#1}}
\newcommand{\tabRef}[1]{Table~\ref{#1}}
\newcommand{\figRef}[1]{Figure~\ref{#1}}
\newcommand{\secRef}[1]{Section~\ref{#1}}
\newcommand{\algRef}[1]{Algorithm~\ref{#1}}

% === Colorization tools ======
\newcommand{\colorstuff}[2]{\color{#1}{#2}\color{black}}

% ==== spacing control on caption =====
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}



==> texlib/ieee_setting.tex <==
% =============================================================
%            setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 06/2015
% =============================================================


%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}    % new algorithm package
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subfigure}
\usepackage{graphicx}         % include pdf figures
\usepackage{color}
\usepackage{cite}             % more citations in one bracket
\usepackage{comment}          % use comment
\usepackage{soul}             % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}         % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}              % nth command
\usepackage{bm}               % bm command


\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myconjecture}{Conjecture}


% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% ==== Logs:
%
%  06/2015: clean IEEEtranBSTCTL commands
%  11/2014: \solregister, to support highlight to mybox, definition, and citations
%  10/2014: add package "authblk" & "bm"
%  09/2014: "problem" => "myproblem"
%  07/2014: introduce \Statex[] for lone algorithmic statement
%  05/2014: new package {soul} to use highlight command \hl{}
%




==> texlib/poster_setting.tex <==
% ============================================================
%             Beamer poster setting file
%
%   Author      : Bei Yu
%   last Update : 06/2014
% ============================================================

% additional settings
\setbeamerfont{itemize}{size=\normalsize}
\setbeamerfont{itemize/enumerate body}{size=\normalsize}
\setbeamerfont{itemize/enumerate subbody}{size=\normalsize}


% block width setting
\newenvironment<>{varblock}[2][\textwidth]{%
  \setlength{\textwidth}{#1}
  \setbeamercolor{block title}{fg=white,bg=blue!20!green}
  %\setbeamercolor{block body}{fg=black,bg=olive!50}
  \setbeamercolor{block body}{fg=black,bg=blue!10}
  \begin{actionenv}#3%
  \def\insertblocktitle{#2}%
  \par%
  \usebeamertemplate{block begin}}
  {
    \par%
    \usebeamertemplate{block end}%
    \end{actionenv}
  }


% abbreviations
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot}
\def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother


% === including packages
\usepackage{bm}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{times}
\usepackage{amsmath,amsthm, amssymb, latexsym}
\usepackage{exscale}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{comment}
\usepackage{booktabs, array}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage[orientation=landscape,size=custom,width=200,height=230,scale=1.9]{beamerposter}
\listfiles

% =====  algorithm setting
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

% ==== Log
%
%  05/2014: preliminary results show that pgf library is NOT good for poster
%


